Matematika 1

The book was written on the basis of materials that we presented at several faculties, either as lectures or as part of auditory exercises. Aware that there are more books and textbooks in the area in which the topics covered by this book are covered, we tried, based on the mentioned experience, to write a book oriented towards students.

==> dodatak.tex <==

\section{D\lowercase{jeljivost cijelih brojeva}}

 Teorija brojeva je grana matematike koja se ponajprije bavi prou\v cavanjem osobina skupa prirodnih brojeva $\mathbb{N}$. Osim toga, prou\v cavaju se i osobine skupa cijelih brojeva $\mathbb{Z},$ te racionalnih brojeva $\mathbb{Q}$. Pojam djeljivosti je jedan od najjednostavnijih, ali i najva\v znijih pojmova u teoriji brojeva. Kada cio broj podijelimo drugim cijelim brojem razli\v citim od nule, rezultat mo\v ze a i ne mora biti cio broj. Na primjer, $32:4=8$ je cio broj, dok $12:5=2.4$ nije cio broj. Ovi primjeri vode nas do sljede\' ce definicije.
\begin{definition}
  Ako su $a$ i $b$ cijeli brojevi i $a\neq 0,$ ka\v zemo da $a$ dijeli $b$ ili da je $b$ djeljivo sa $a,$ ako postoji cio broj $c,$ takav da je $b=a\cdot c.$ Ako $a$ dijeli $b,$ ka\v zemo $a$ je djelilac ili faktor od broja $b.$
\end{definition}

Ako $a$ dijeli $b$ pi\v semo $a\mid b,$ a ako ne dijeli onda $a\nmid b.$
\begin{example}
  Sljede\' ci primjeri ilustruju koncept djeljivosti cijelih brojeva: $7\mid 35,\:13\mid 65,\:11\mid 55,\:-5\mid 45,\:14\mid 0,\:3\nmid 10,\:4\nmid 17.$
\end{example}

\begin{example}
  Djelioci broja $6$ su $\pm 1,\:\pm 2,\:\pm 3,\:\pm 6.$ Djelioci broja $19$ su $\pm 1$ i $\pm 19.$ Djelioci broja $100$ su\\ $\pm 1,\,\pm 2,\, \pm 4,\,\pm 5,\,\pm 10,\,\pm 20,\,\pm 25,\, \pm 50$ i $\pm 100.$
\end{example}


Slijede neke osnovne osobine djeljivosti.

\begin{theorem}\label{djeljivost1}
  Ako su $a,\,b$ i $c$ cijeli brojevi takvi da je $a\mid b$ i $b\mid c,$ tada je $a\mid c.$
\end{theorem}

\begin{example}
  Ako je $7\mid 35$ i $35\mid 105,$ tada po Teoremi  \ref{djeljivost1} slijedi da je $7\mid 105.$
\end{example}

\begin{theorem}\label{djeljivost2}
   Ako je su $a,\,b,\,c,\,m$ i $n$ cijeli brojevi takvi da je $c\mid a,\,c\mid b,$ tada je $c\mid (ma+nb).$
\end{theorem}

\begin{example}
  Kako je $3\mid 12$ i $3\mid 21,$ tada po Teoremi \ref{djeljivost2}, $3$ dijeli i $39$ jer je
  \[5\cdot 12-1\cdot 21=39.\]
\end{example}

\begin{theorem}[Teorema o dijeljenju sa ostatkom]
   Ako su $a$ i $b,\,b>0$ cijeli brojevi, tada postoje jedinstveni cijeli brojevi $q$ i $r$ takvi da je
   \[a=b\cdot q+r \text{  i  } 0\leqslant r<b.\]
\end{theorem}

U prethodnoj teoremi broj $a$ je dijeljenik, $b$ je djelilac, $q$ je koli\v cnik i  $r$ je ostatak. Ova teorema se negdje naziva i algoritam dijeljenja. Iz $a=bq+r$ mo\v zemo primijetiti da je $a$ djeljivo sa $b$ jedino ako je $r=0.$


\begin{example}
  Ako je $a=133$ i $b=21$, tada je $q=6$  i $r=7,$ jer je $133=21\cdot 6+7.$% Vrijedi i $a=-50,\,b=8,\,q=-7,\,r=6,$ jer je $-50=-7\cdot 8+6.$
\end{example}





Za dati pozitivan cio broj $d,$ mo\v zemo cijele brojeve svrstati u razli\v cite podskupove zavisno od toga koliki je ostatak nekog cjelog broja pri dijeljenju sa $d$. Ako je broj $d=2$ onda su mogu\' ci ostaci $0$ i $1.$ Ovo nas vodi do sljede\' ce definicije.

\begin{definition}
  Ako je ostatak dijeljenja cijelog pozitivnog broja $n$ sa $2$ jednak $0,$ tada je $n=2k$ za neki pozitivan cio broj $k$ i ka\v zemo da je $n$ paran broj. U suprotnom, ako je ostatak dijeljenja $n$ sa $2$ jednak $1,$ onda je $n=2k+1,$ za neki pozitivan cio broj $k$ i ka\v zemo da je $n$ neparan broj.
\end{definition}


\paragraph{Prosti i slo\v zeni brojevi}

Broj $1$ ima samo jednog pozitivnog djelioca i to je $1.$ Svaki drugi pozitivan cio broj ima najmanje dva pozitivna djelioca i to $1$ i samog sebe. Pozitivni cijeli brojevi koji imaju samo dva djelioca jako su bitni.

\begin{definition}[Prosti brojevi]
    Prost broj je pozitivan cio broj koji je djeljiv jedino sa $1$  i samim sobom.
\end{definition}

\begin{example}
  Prosti brojevi su $2,\,3,\,5,\,7,\,11,\, 13, \ldots$
\end{example}

\begin{definition}[Slo\v zeni brojevi]
   Pozitivni cijeli brojevi ve\' ci od $1$ koji nisu prosti nazivaju se slo\v zeni brojevi.
\end{definition}

\begin{example}
  Slo\v zeni brojevi su $12=2\cdot 2\cdot 3,\,15=3\cdot 5,\,60=2\cdot 2\cdot  3\cdot 5,\ldots$
\end{example}


Vrijedi teorema.
\begin{theorem}[Euklidov teorem]
Prostih brojeva ima beskona\v cno mnogo.
\end{theorem}
\begin{proof}[Dokaz]
Pretpostavimo da prostih brojeva ima kona\v cno mnogo i da su to $p_1,\ldots,p_{k-1},p_k,p_{k+1},\ldots,p_n.$ Konstrui\v simo sljede\' ci broj $q=p_1\cdot\ldots \cdot p_{k-1}\cdot p_k\cdot p_{k+1}\cdot\ldots\cdot p_n+1,$ ovaj broj je po na\v soj pretpostavci slo\v zen, jer su samo $p_1,\ldots,p_{k-1},p_k,p_{k+1},\ldots, p_n$ prosti brojevi.  Po\v sto je $q$ slo\v zen broj, mora postojati njegov djelioc razli\v cit od $1$ i njega samog. Podijelimo broj $q$ bilo kojim prostim brojem, na primjer sa $p_k,$ vrijedi
\[\frac{q}{p_k}=\frac{p_1\cdot\ldots \cdot p_{k-1}\cdot p_k\cdot p_{k+1}\cdot\ldots\cdot p_n+1}{p_k}
 =p_1\cdot\ldots \cdot p_{k-1}\cdot p_{k+1}\cdot\ldots\cdot p_n+\frac{1}{p_k}.\] Dobijeni broj nije cio (racionalan broj bi dobili u slu\v caju dijeljenja sa bilo kojim od brojeva $p_1,\ldots,p_n$), pa $q$ nije djeljiv ni sa jednim prostim brojem, tj. $q$ je i sam prost broj. Proces konstruisanja brojeva na na\v cin kako je konstruisan broj $q$ mo\v zemo nastaviti proizvoljan broj puta. Dakle pretpostavka da prostih brojeva ima kona\v cno mnogo je pogre\v sna.
\end{proof}


Fundametalna teorema aritmetike je va\v zan rezultat, koji ka\v ze da su prosti brojevi fundamentalni blokovi za izgradnju slo\v zenih brojeva.
\begin{theorem}[Fundamentalni teorem aritmetike]\label{fundamentalnith}
   Svaki slo\v zeni broj mo\v ze biti predstavljen na jedinstven na\v cin kao proizvod prostih brojeva, pri \v cemu su prosti brojevi u proizvodu zapisani u neopadaju\' cem redoslijedu.
\end{theorem}
\begin{example}
   Brojeve $12,\,30,\,33,\,48,$ zapisujemo na sljede\' ci na\v cin:
   \[12=2^2\cdot 3,\:30=2\cdot3\cdot 5,\:33=3\cdot 11,\:48=2^4\cdot 3.\]
\end{example}



\subsection{Najve\' ci zajedni\v cki djelilac i najmanji zajedni\v cki  sadr\v zilac}

Neka su $a$ i $b$ cijeli brojevi, razli\v citi od nule, tada je skup zajedni\v ckih djelilaca brojeva $a$ i $b$ neki kona\v can skup cijelih brojeva koji uvijek sadr\v zi $-1$ i $1.$ Zanima nas koji je najve\' ci djelilac ova dva broja $a$ i $b.$

\begin{definition}[Najve\' ci zajedni\v cki djelilac]
  Najve\' ci zajedni\v cki djelilac cijelih brojeva $a$ i $b,$ razli\v citih od nule, je najve\' ci djelilac koji dijeli istovremeno i $a$ i $b.$
\end{definition}
Najve\' ci zajedni\v cki djelilac brojeva $a$ i $b$ ozna\v cavamo sa $\nzd(a,b),$ (ili $(a,b)$). Broj $0$ ima beskona\v cno mnogo djelilaca. 

\begin{example}
  Zajedni\v cki djelioci brojeva $24$ i $84$ su: $\pm 1,\,\pm 2,\,\pm 3,\, \pm 4,\,\pm 6$ i $\pm 12.$ Dakle $\nzd(24,84)=12.$ Vrijedi i $\nzd(15,81)=3,\,\nzd(100,5)=5,\,\nzd(17,25)=1,\,\nzd(0,44)=44,\,\nzd(-15,-6)=3$ i $\nzd(-17,289)=17.$
\end{example}
Ako je najve\' ci zajedni\v cki djelilac dva cijela broja $a$ i $b$ jednak $1$ tada taj par ima posebno ime.
\begin{definition}[Relativno prosti brojevi]
  Cijeli brojevi $a$ i $b$ su relativno prosti ako je najve\' ci zajedni\v cki djelilac ova dva broja $1,$ tj. $\nzd(a,b)=1.$
\end{definition}

\begin{example}
 Kako je $\nzd(25,42)=1,$ to su $25$ i $42$ relativno prosti.
\end{example}


\paragraph{Euklidov algoritam}
Euklidov algoritam predstavlja sistematski metod za ra\v cunanje najve\' ceg zajedni\v ckog djelioca dva cijela broja $a$ i $b$ bez direktnog ra\v cunanja zajedni\v ckih djelilaca. Ime je dobio po gr\v ckom matemati\v caru Euklidu\footnote{Euclid (ro\dj en sredinom 4. vijeka p.n.e, umro sredinom 3. vijeka p.n.e), napisao Elemente-djelo od 13 knjiga, jedno od najuticajnijih djela u razvoju matematike}.



\begin{theorem}[Euklidov algoritam]
  Neka su $r_0=a$ i $r_1=b$ cijeli brojevi takvi da je $a\geqslant b>0.$ Ako algoritam dijeljenja sukscesivno primijenimo da dobijemo $r_j=r_{j+1}q_{j+1}+r_{j+2}$ gdje je $0<r_{j+2}<r_{r+1}$ za $j=0,1,\ldots,n-2$ i $r_{n+1}=0$ tada je $\nzd(a,b)=r_n,$ tj. zadnji  ostatak razli\v cit od nule je najve\' ci zajedni\v cki djelilac brojeva $a$ i $b.$
\end{theorem}

\begin{example}
   Odrediti \\
      \begin{inparaenum}
         \item $\nzd(252,198).\:$\\
         \item $\nzd(102,222).\:$
      \end{inparaenum}\\
Rje\v senje:
  \begin{enumerate}
  \item    \begin{align*}
      252=&1\cdot 198+54\\
      198=&3\cdot 54+36\\
      54=&1\cdot 36+{\color{magenta}18}\\
      36=&2\cdot 18,
   \end{align*}
   pa je $\nzd(252,198)=18.$
   \item
     \begin{align*}
        222=&2\cdot 102+18\\
        102=& 5\cdot 18+12\\
        18=&1\cdot 12+{\color{magenta}6}\\
        12=&2\cdot 6,
   \end{align*}
pa je $\nzd(222,102)=6.$
\end{enumerate}
\end{example}

\paragraph{Najmanji zajedni\v cki sadr\v zilac}

Faktorizacija na proste brojeve mo\v ze biti iskori\v stena za ra\v cunanje najmanjeg cijelog pozitivnog broja koji sadr\v zi dva pozitivna cijela broja. Na ovaj problem nailazimo, na primjer, prilikom sabiranja razlomaka.
\begin{definition}[Najmanji zajedni\v cki sadr\v zilac]
  Najmanji zajedni\v cki sadr\v zilac pozitivnih cijelih brojeva $a$ i $b$ je najmanji pozitivan broj koji je djeljiv i sa $a$ i sa $b.$
\end{definition}
Najmanji zajedni\v cki sadr\v zilac brojeva $a$ i $b$ ozna\v cavamo sa $\nzs(a,b)$ (ili sa $[a,b]$).



\begin{example}
  Koriste\' ci faktorizaciju na proste brojeve izra\v cunati $\nzd(90,24)$ i $ \nzs(90,24).$\\\\
Rje\v senje. Izvr\v simo prvo faktorizaciju brojeva $90$ i $24.$ Dijelimo brojeve $90$ i $ 24$ prostim brojevima po\v cev od $2,\,3,\,\ldots,$ ako su brojevi $90$ i $24$ djeljivi pi\v semo rezultat. Vrijedi
\begin{align*}
       90&=45\cdot 2 & 24&=12\cdot 2\\
       45&=15\cdot 3 & 12&=6\cdot 2\\
       15&=5\cdot 3  & 6&=3\cdot 2\\
       5&=1\cdot 5   & 3&=1\cdot 3,
\end{align*}
pa je
\begin{align*}
    90&=2\cdot 3\cdot 3\cdot 5\\
    24&=2\cdot 2\cdot 2\cdot 3.
\end{align*}

Iz oba razvoja biramo zajedni\v cke faktore, to su $2$ i $3.$ Njihov proizvod je najve\' ci zajedni\v cki djelilac brojeva $90$ i $24,$ tj. $\nzd(90,24)=2\cdot 3=6.$

Najmanji zajedni\v cki sadr\v zilac dobijamo tako \v sto uzimamo sve faktore koji se pojavljuju u oba razvoja, ali bez ponavljanja. Iz drugog razvoja uzimamo proizvod $2\cdot 2\cdot 2,$ broj $2$ iz razvoja broja $90$ ne\' cemo uzimati jer ve\' c imamo $2$ u proizvodu $2\cdot 2\cdot 2,$ zatim uzimamo proizvod $3\cdot 3$ iz prvog razvoja, opet ne\' cemo uzeti $3$ iz drugog razvoja jer smo ve\' c uzeli $3\cdot 3$ i na kraju uzimamo $5$ u proizvod, pa je $\nzs(90,24)=2\cdot 2\cdot 2\cdot 3\cdot 3\cdot 5=360.$
\end{example}



\section{Z\lowercase{adaci}}\index{Zadaci za vje\v zbu!djeljivost cijelih brojeva}
	
 \begin{enumerate}
 	\item Primjenjuju\'ci algoritam dijeljenja, odrediti brojeve $q$ i $r$ tako da je $a=b\cdot q+r,$ ako je    \\
 	      \begin{inparaenum}
 	      	\item $a=18,$ $b=4;$
 	      	\item $a=65,$ $b=9;$
 	      	\item $a=763,$ $b=24;$
 	      	\item $a=1000,$ $b=143.$
 	      \end{inparaenum}

    \item   Odrediti najve\'ci zajedni\v cki djelilac $\nzd$ \\
         \begin{inparaenum}
         	\item $\nzd(12,15);$
         	\item $\nzd(9,21);$
         	\item $\nzd(24, 60);$
         	\item $\nzd(52,76);$
         	
         	\item $\nzd(13,25);$
         	\item $\nzd(225, 102);$
         	\item $\nzd(524, 88);$
         	\item $\nzd(1331,1001).$          	
         \end{inparaenum}

     \item Odrediti najmanji zajedni\v cki sadr\v zilac $\nzs$ \\
        \begin{inparaenum}
        	\item  $\nzs(6,15 );$
        	\item  $\nzs(7,12 );$
        	\item  $\nzs(9,24 );$
        	\item  $\nzs(10, 48 );$
        	
        	\item  $\nzs(15,24 );$
        	\item  $\nzs(32, 92 );$
        	\item  $\nzs(54, 216 );$
        	\item  $\nzs(42, 200 ).$
        \end{inparaenum}


 \end{enumerate}	









==> naslovB5.tex <==

%----------------------------------------------------------------------------------------
%	TITLE PAGE
%----------------------------------------------------------------------------------------

\begin{titlepage} % Suppresses displaying the page number on the title page and the subsequent page counts as page 1
	\newcommand{\HRule}{\rule{\linewidth}{0.125mm}} % Defines a new command for horizontal lines, change thickness here
	
	\center % Centre everything on the page
	
	%------------------------------------------------
	%	Headings
	%------------------------------------------------
	
 {\Large  Samir Karasulji\'c \quad  Sanela Halilovi\'c  }\\[1.5cm] % Main heading such as the name of your university/college
	
	%\textsc{\Large  }\\[0.5cm] % Major heading such as course name
	
	%\textsc{\large }\\[0.5cm] % Minor heading such as course title
	
	%------------------------------------------------
	%	Title
	%------------------------------------------------
	
	\HRule\\[0.4cm]
	
	{\huge\bfseries Matematika 1}\\[0.0cm] % Title of your document
	
	\HRule
\ \\[1.5cm]
	\large za studente hemije, tehnologije, razredne nastave i pred\v skolskog odgoja  \\[0.5cm] % Minor heading such as course title



	%------------------------------------------------
	%	Author(s)
	%------------------------------------------------
%	 \vspace{2cm}
%	\begin{minipage}{0.4\textwidth}%
%		\begin{flushleft}
%			\large
%			\textit{Autori}\\
%			Samir Karasulji\' c\\
%			Sanela Halilovi\'c
%			\textsc{ } \\ % Your name
%		\end{flushleft}
%	\end{minipage}
%	~
%	\begin{minipage}{0.4\textwidth}
%		\begin{flushleft}\vspace{1cm}
%			\large
%			Email \texttt{samir.karasuljic@unitz.ba}\\
%                  \texttt{samir.karasuljic@gmail.com}\\ 
%                  \texttt{sanela.halilovic@unitz.ba}\\
%                  \texttt{halilovicsanela8@gmail.com} %
%			% \textsc{ } % Supervisor's name
%		\end{flushleft}
%	\end{minipage}
	
	% If you don't want a supervisor, uncomment the two lines below and comment the code above
	%{\large\textit{Author}}\\
	%John \textsc{Smith} % Your name
	
	%------------------------------------------------
	%	Date
	%------------------------------------------------
	
	\vfill\vfill\vfill % Position the date 3/4 down the remaining page
	
	{Tuzla, 2021. godina} % Date, change the \today to a set date if you want to be precise
	
	%------------------------------------------------
	%	Logo
	%------------------------------------------------
	
	%\vfill\vfill
	%\includegraphics[width=0.2\textwidth]{placeholder.jpg}\\[1cm] % Include a department/university logo - this will require the graphicx package
	 
	%----------------------------------------------------------------------------------------
	
	\vfill % Push the date up 1/4 of the remaining page
	
\end{titlepage}

%----------------------------------------------------------------------------------------
